Credible, Strategyproof, Optimal, and Bounded Expected-Round Single-Item Auctions for all Distributions

We consider a revenue-maximizing seller with a single item for sale to multiple buyers with i.i.d. valuations. Akbarpour and Li (2020) show that the only optimal, credible, strategyproof auction is the ascending price auction with reserves which has unbounded communication complexity. Recent work of Ferreira and Weinberg (2020) circumvents their impossibility result assuming the existence of cryptographically secure commitment schemes, and designs a two-round credible, strategyproof, optimal auction. However, their auction is only credible when buyers' valuations are MHR or $\alpha$-strongly regular: they show their auction might not be credible even when there is a single buyer drawn from a non-MHR distribution. In this work, under the same cryptographic assumptions, we identify a new single-item auction that is credible, strategyproof, revenue optimal, and terminates in constant rounds in expectation for all distributions with finite monopoly price.

==> E-two-rounds.tex <==
\newpage
\section{Results for Two Rounds}\label{app:tworounds}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
When there's two bidders with interleaved values, and value sets of size two each, then a credible mechanism needs two rounds.
\end{lemma}

\begin{proof}
We assume for contradiction that there is a single round protocol that resolves the auction. Let Alice have value set $\{x_1, x_2\}$ and Bob have values $\{y_1, y_2\}$, such that $x_1 < y_1 < x_2 < y_2$.  Now consider the following scenario where Alice has value $x_1$ and Bob has value $y_2$. Then the auctioneer can lie and tell Bob that Alice has value $x_2$. This gets strictly more revenue.  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma} When there's two bidders with interleaved values, and value sets $A$ and $B$, then a credible mechanism needs $\min\{|A|,|B|\}$ rounds. \end{lemma}

%\begin{proof} Induction? \end{proof}

\begin{lemma}
A mechanism is strategy-proof if and only if for each bidder $i$, $p_i(v_i, \vec{v}_{-i}) = p_i(v'_i, \vec{v}_{-i})$.
\end{lemma}

\begin{proof}
Assume that in the last round, there exists some bidder $i$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v'_i, \vec{v}_{-i})$. We consider the scenario where $p_i(v_i, \vec{v}_{-i}) < p_i(v'_i, \vec{v}_{-i})$ and bidder $i$'s value is $v'_i$. Here, bidder $i$ pays strictly less by not being truthful and saying she has value $v_i$, which contradicts strategy-proofness.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
A mechanism is credible if and only if in the last round, for each bidder $i$, $p_i(v_i, \vec{v}_{-i}) = p_i(v_i, \vec{v}'_{-i})$.
\end{lemma}

\begin{proof}
Assume that in the last round, there exists some bidder $i$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v_i, \vec{v}'_{-i})$. We consider the scenario where $p_i(v_i, \vec{v}_{-i}) < p_i(v_i, \vec{v}'_{-i})$ and the other bidders' values are $\vec{v}_{-i}$. Here, the auctioneer gets strictly more revenue by not being truthful and saying that the other other bidders' values are $\vec{v'}_{-i}$, which contradicts credibility.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
The last round is strategy-proof and credible if and only if it is posted-price.
\end{lemma}

\begin{proof}
We first prove that if the last round is posted price then it is strategy-proof and credible. Consider what happens in the case where we assume the last round is not strategy-proof. Then there exists bidder $i$ and two distinct values $v_i, v'_i$ drawn from $V_i$ and $\vec{v}_{-i}$ drawn from $V_{-i}$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v'_i, \vec{v}_{-i})$. Thus, bidder $i$ can win with two different prices even when all other values $\vec{v}_{-i}$ are fixed.
This contradicts posted-price.

Now consider what happens in the case where we assume that the last round is not credible. Then there exists bidder $i$ with $v_i$ drawn from $V_i$ and two vectors $\vec{v}_{-i}, \vec{v}'_{-i}$ drawn from $V_{-i}$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v_i, \vec{v}'_{-i})$. Thus, bidder $i$ can win with two different prices for the same fixed value $v_{i}$. This also contradicts posted-price.
We can therefore conclude that if the last round is posted price then it is strategy-proof and credible.

We now prove that if the last round is  strategy-proof and credible then it is posted-price.
Consider what happens when we assume the mechanism is not posted price.  Then there exists $\vec{v}, \vec{v}'$ drawn from $V$, where bidder $i$ wins with values $v_i$ and $v'_i$. We let $p_i(v_i, \vec{v}_{-i}) < p_i(v_i',\vec{v}'_{-i})$. \hide{, and let $v_j$ and $v'_j$ be the second highest bids in $v$ and $v'$ respectively.} We now have two cases.

Consider what happens in the first case where we $v_i < v'_i$. We define the value vector $\hat{v} = (v'_i, \vec{v}_{-i})$. Bidder $i$ is still the winner under $\hat{v}$ because $v'_i>v_i>\vec{v}_{-i}$. But since this is strategy-proof, we have $p_i(\hat{v}) = p_i(v'_i, \vec{v}_{-i}) = p_i(v_i, \vec{v}_{-i}) = p_i(\vec{v}) < p_i(\vec{v}')$. Thus, bidder $i$ can win with two different prices $p_i(v'_i, \vec{v}_{-i}) < p_i(v'_i, \vec{v}'_{-i})$ for the same value $v'_i$. This contradicts credibility.

Now consider what happens in the second case where we have $v_i > v'_i$. We define the value vector $\hat{v} = (v_i, \vec{v}'_{-i})$. Bidder $i$ is still the winner because $v_i>v'_i>\vec{v}'_{-i}$. But since this is credible, we have $p_i(\hat{v}) = p_i(v_i, \vec{v}'_{-i}) = p_i(v_i, \vec{v}_{-i}) = p_i(\vec{v}) < p_i(\vec{v}')$. Thus, bidder $i$ can win with two different prices $p_i(v_i, \vec{v}'_{-i}) < p_i(v'_i, \vec{v}'_{-i})$ even when all others bidders' values are fixed to  $\vec{v}'_{-i}$. This contradicts strategy-proofness.
We can therefore conclude that if the last round is strategy-proof and credible then it is posted-price.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:twobidders-inter}
When there are two bidders with interleaved values, only the bidder with the highest possible remaining value $v^*$ in the last round, can pool $v^*$ with another value. The other bidder has a singleton $\{v_2\}$ in the last round. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Assume the values are interleaved, and let $v^*$ denote the highest remaining value among all bidders in the last round. Define $j$ to be the bidder with value $v^*$ in her value set, and let $i$ denote the other bidder.
We now assume for contradiction that two values $\{v, w\}$ both not equal to $v^*$ are pooled together. We have $v < v^*$ and $w < v^*$, so there exists a value $u$ that the other bidder $j$ has, such that $u>v$ and $u>w$.

Now consider the scenario where bidder $i$'s value is $w$ and bidder $j$'s value is $u$. Then in the first round, bidder $i$ says the action that pools $v$ and $w$ together, and bidder $j$ says the action which contains $u$. In the last round, bidder $i$ will say $w$, and bidder $j$ will say $u$.
However, the auctioneer can lie and tell bidder $j$ that bidder $i$ said $v$ ($>w$ and $>u$). This gets strictly more revenue, so the mechanism is not credible.\\
Therefore, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
When there are $n$ bidders with interleaved values, the bidder with the highest possible value $v^*$ can pool $v^*$ with another value in the last round, and a strong guaranteed losing bidder (if one exists) with the two lowest possible values $v_{\min_1}$ and $v_{\min_2}$ can pool those two values. The other bidders have a singleton $\{v_i\}$ in the last round. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Suppose there exists two values $v$ and $w$ both not equal to $v^*, v_{\min_1}, v_{\min_2}$, and that are pooled together by any bidder $i$. We have $v < v^*$ and $w < v^*$, so there exists a value $u$ that some other bidder $j$ has, such that $u>v$ and $u>w$.

Now consider the scenario where bidder $i$'s value is $w$ and bidder $j$'s value is $u$. Then in the first round, bidder $i$ says the action that pools $v$ and $w$ together, and bidder $j$ says the action which contains $u$. In the last round, bidder $i$ will say $w$, and bidder $j$ will say $u$.

However, the auctioneer can lie and tell bidder $j$ that bidder $i$ said $v$ ($>w$ and $>u$). This gets strictly more revenue, so the mechanism is not credible.
Therefore, no two values both $\neq v^*, v_{\min_1}, v_{\min_2}$ can be pooled together in the second-to-last round.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}[Updated lemma~\ref{lem:twobidders-inter}]
Let $v^*$ be the biggest value among all the values of the two bidders, and let $j$ denote the bidder with possible value $v^*$. Then bidder $\neq j$ must be a singleton. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Consider what happens when the auctioneer learns that bidder $j$ has value $v^*$. Then bidder $j$ certainly wins, and the auctioneer tells bidder $j$ that the other bidder has the highest possible remaining value (which makes them pay strictly the most, since values are interleaved for the two bidders).

Now assume for contradiction that two values $\{v, w\}$ both $\neq v^*$ are pooled together. Since neither is $v^*$ and the values are interleaved, there exists a value $u$ of the other bidder $> \{v, w\}$.

Now consider the scenario where this bidder has value $w$ and the other bidder does have value $u$. Then in the first round, this bidder says the action which pools $v$ and $w$ together, and the other bidders says the action which contains $u$. Then, in the last round, the other bidder will announce $u$. When this bidder announces $w$, the auctioneer can lie and pretend they said $v$ (instead of $w < v$). This gets them strictly more revenue.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[credible]
Auctioneer has no profitable deviation.\\
Bidder one: $10$ and $7$\\
Bidder two: $8$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[credible]
Auctioneer has no profitable deviation. Not strategyproof?\\
Bidder one: $10$ and $8$\\
Bidder two: $7$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[credible]
Auctioneer has no profitable deviation.\\
Bidder one: $10$\\
Bidder two: $8$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[not credible]
Auctioneer can tell bidder one that bidder two has value $5$ always.\\
Bidder one: $10$\\
Bidder two: $5$ and $4$\\
Bidder three: $1$
\end{example}

\begin{example}[not credible]
Auctioneer can tell bidder one that bidder two has value $7$ always.\\
Bidder one: $10$ and $8$\\
Bidder two: $7$ and $4$\\
Bidder three: $5$
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> F-two-rounds.tex <==
\newpage
\section{Results for Two Rounds}\label{app:tworounds}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
When there's two bidders with interleaved values, and value sets of size two each, then a credible mechanism needs two rounds.
\end{lemma}

\begin{proof}
We assume for contradiction that there is a single round protocol that resolves the auction. Let Alice have value set $\{x_1, x_2\}$ and Bob have values $\{y_1, y_2\}$, such that $x_1 < y_1 < x_2 < y_2$.  Now consider the following scenario where Alice has value $x_1$ and Bob has value $y_2$. Then the auctioneer can lie and tell Bob that Alice has value $x_2$. This gets strictly more revenue.  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma} When there's two bidders with interleaved values, and value sets $A$ and $B$, then a credible mechanism needs $\min\{|A|,|B|\}$ rounds. \end{lemma}

%\begin{proof} Induction? \end{proof}

\begin{lemma}
A mechanism is strategy-proof if and only if for each bidder $i$, $p_i(v_i, \vec{v}_{-i}) = p_i(v'_i, \vec{v}_{-i})$.
\end{lemma}

\begin{proof}
Assume that in the last round, there exists some bidder $i$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v'_i, \vec{v}_{-i})$. We consider the scenario where $p_i(v_i, \vec{v}_{-i}) < p_i(v'_i, \vec{v}_{-i})$ and bidder $i$'s value is $v'_i$. Here, bidder $i$ pays strictly less by not being truthful and saying she has value $v_i$, which contradicts strategy-proofness.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
A mechanism is credible if and only if in the last round, for each bidder $i$, $p_i(v_i, \vec{v}_{-i}) = p_i(v_i, \vec{v}'_{-i})$.
\end{lemma}

\begin{proof}
Assume that in the last round, there exists some bidder $i$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v_i, \vec{v}'_{-i})$. We consider the scenario where $p_i(v_i, \vec{v}_{-i}) < p_i(v_i, \vec{v}'_{-i})$ and the other bidders' values are $\vec{v}_{-i}$. Here, the auctioneer gets strictly more revenue by not being truthful and saying that the other other bidders' values are $\vec{v'}_{-i}$, which contradicts credibility.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
The last round is strategy-proof and credible if and only if it is posted-price.
\end{lemma}

\begin{proof}
We first prove that if the last round is posted price then it is strategy-proof and credible. Consider what happens in the case where we assume the last round is not strategy-proof. Then there exists bidder $i$ and two distinct values $v_i, v'_i$ drawn from $V_i$ and $\vec{v}_{-i}$ drawn from $V_{-i}$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v'_i, \vec{v}_{-i})$. Thus, bidder $i$ can win with two different prices even when all other values $\vec{v}_{-i}$ are fixed.
This contradicts posted-price.

Now consider what happens in the case where we assume that the last round is not credible. Then there exists bidder $i$ with $v_i$ drawn from $V_i$ and two vectors $\vec{v}_{-i}, \vec{v}'_{-i}$ drawn from $V_{-i}$ such that $p_i(v_i, \vec{v}_{-i}) \neq p_i(v_i, \vec{v}'_{-i})$. Thus, bidder $i$ can win with two different prices for the same fixed value $v_{i}$. This also contradicts posted-price.
We can therefore conclude that if the last round is posted price then it is strategy-proof and credible.

We now prove that if the last round is  strategy-proof and credible then it is posted-price.
Consider what happens when we assume the mechanism is not posted price.  Then there exists $\vec{v}, \vec{v}'$ drawn from $V$, where bidder $i$ wins with values $v_i$ and $v'_i$. We let $p_i(v_i, \vec{v}_{-i}) < p_i(v_i',\vec{v}'_{-i})$. \hide{, and let $v_j$ and $v'_j$ be the second highest bids in $v$ and $v'$ respectively.} We now have two cases.

Consider what happens in the first case where we $v_i < v'_i$. We define the value vector $\hat{v} = (v'_i, \vec{v}_{-i})$. Bidder $i$ is still the winner under $\hat{v}$ because $v'_i>v_i>\vec{v}_{-i}$. But since this is strategy-proof, we have $p_i(\hat{v}) = p_i(v'_i, \vec{v}_{-i}) = p_i(v_i, \vec{v}_{-i}) = p_i(\vec{v}) < p_i(\vec{v}')$. Thus, bidder $i$ can win with two different prices $p_i(v'_i, \vec{v}_{-i}) < p_i(v'_i, \vec{v}'_{-i})$ for the same value $v'_i$. This contradicts credibility.

Now consider what happens in the second case where we have $v_i > v'_i$. We define the value vector $\hat{v} = (v_i, \vec{v}'_{-i})$. Bidder $i$ is still the winner because $v_i>v'_i>\vec{v}'_{-i}$. But since this is credible, we have $p_i(\hat{v}) = p_i(v_i, \vec{v}'_{-i}) = p_i(v_i, \vec{v}_{-i}) = p_i(\vec{v}) < p_i(\vec{v}')$. Thus, bidder $i$ can win with two different prices $p_i(v_i, \vec{v}'_{-i}) < p_i(v'_i, \vec{v}'_{-i})$ even when all others bidders' values are fixed to  $\vec{v}'_{-i}$. This contradicts strategy-proofness.
We can therefore conclude that if the last round is strategy-proof and credible then it is posted-price.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:twobidders-inter}
When there are two bidders with interleaved values, only the bidder with the highest possible remaining value $v^*$ in the last round, can pool $v^*$ with another value. The other bidder has a singleton $\{v_2\}$ in the last round. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Assume the values are interleaved, and let $v^*$ denote the highest remaining value among all bidders in the last round. Define $j$ to be the bidder with value $v^*$ in her value set, and let $i$ denote the other bidder.
We now assume for contradiction that two values $\{v, w\}$ both not equal to $v^*$ are pooled together. We have $v < v^*$ and $w < v^*$, so there exists a value $u$ that the other bidder $j$ has, such that $u>v$ and $u>w$.

Now consider the scenario where bidder $i$'s value is $w$ and bidder $j$'s value is $u$. Then in the first round, bidder $i$ says the action that pools $v$ and $w$ together, and bidder $j$ says the action which contains $u$. In the last round, bidder $i$ will say $w$, and bidder $j$ will say $u$.
However, the auctioneer can lie and tell bidder $j$ that bidder $i$ said $v$ ($>w$ and $>u$). This gets strictly more revenue, so the mechanism is not credible.\\
Therefore, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
When there are $n$ bidders with interleaved values, the bidder with the highest possible value $v^*$ can pool $v^*$ with another value in the last round, and a strong guaranteed losing bidder (if one exists) with the two lowest possible values $v_{\min_1}$ and $v_{\min_2}$ can pool those two values. The other bidders have a singleton $\{v_i\}$ in the last round. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Suppose there exists two values $v$ and $w$ both not equal to $v^*, v_{\min_1}, v_{\min_2}$, and that are pooled together by any bidder $i$. We have $v < v^*$ and $w < v^*$, so there exists a value $u$ that some other bidder $j$ has, such that $u>v$ and $u>w$.

Now consider the scenario where bidder $i$'s value is $w$ and bidder $j$'s value is $u$. Then in the first round, bidder $i$ says the action that pools $v$ and $w$ together, and bidder $j$ says the action which contains $u$. In the last round, bidder $i$ will say $w$, and bidder $j$ will say $u$.

However, the auctioneer can lie and tell bidder $j$ that bidder $i$ said $v$ ($>w$ and $>u$). This gets strictly more revenue, so the mechanism is not credible.
Therefore, no two values both $\neq v^*, v_{\min_1}, v_{\min_2}$ can be pooled together in the second-to-last round.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}[Updated lemma~\ref{lem:twobidders-inter}]
Let $v^*$ be the biggest value among all the values of the two bidders, and let $j$ denote the bidder with possible value $v^*$. Then bidder $\neq j$ must be a singleton. In other words, no two values both $\neq v^*$ can be pooled together in the second-to-last round.
\end{lemma}

\begin{proof}
Consider what happens when the auctioneer learns that bidder $j$ has value $v^*$. Then bidder $j$ certainly wins, and the auctioneer tells bidder $j$ that the other bidder has the highest possible remaining value (which makes them pay strictly the most, since values are interleaved for the two bidders).

Now assume for contradiction that two values $\{v, w\}$ both $\neq v^*$ are pooled together. Since neither is $v^*$ and the values are interleaved, there exists a value $u$ of the other bidder $> \{v, w\}$.

Now consider the scenario where this bidder has value $w$ and the other bidder does have value $u$. Then in the first round, this bidder says the action which pools $v$ and $w$ together, and the other bidders says the action which contains $u$. Then, in the last round, the other bidder will announce $u$. When this bidder announces $w$, the auctioneer can lie and pretend they said $v$ (instead of $w < v$). This gets them strictly more revenue.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}[credible]
Auctioneer has no profitable deviation.\\
Bidder one: $10$ and $7$\\
Bidder two: $8$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[credible]
Auctioneer has no profitable deviation. Not strategyproof?\\
Bidder one: $10$ and $8$\\
Bidder two: $7$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[credible]
Auctioneer has no profitable deviation.\\
Bidder one: $10$\\
Bidder two: $8$\\
Bidder three: $5$ and $4$
\end{example}

\begin{example}[not credible]
Auctioneer can tell bidder one that bidder two has value $5$ always.\\
Bidder one: $10$\\
Bidder two: $5$ and $4$\\
Bidder three: $1$
\end{example}

\begin{example}[not credible]
Auctioneer can tell bidder one that bidder two has value $7$ always.\\
Bidder one: $10$ and $8$\\
Bidder two: $7$ and $4$\\
Bidder three: $5$
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> itcs-macros.tex <==
% Author's notes
\definecolor{DarkRed}{rgb}{0.5,0.1,0.1}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\newcommand{\authnote}[2]{{ \footnotesize \bf{\color{DarkRed}[#1's Note:
{\color{DarkBlue}#2}]}}}

\newcommand{\me}[1]{{\authnote{Meryem} {#1}}}
\newcommand{\mattnote}[1]{{\authnote{Matt} {#1}}}
\newcommand{\madd}[1]{{\color{blue} #1}}
\newcommand{\mc}[1]{{\color{red}MVXF: #1}}
\newcommand{\mattfootnote}[1]{\footnote{\textcolor{blue}{#1}}}
\newcommand{\hide}[1]{}

% Math symbols
\newcommand{\rev}{\text{Rev}}
\newcommand{\vvalue}{\varphi}
\newcommand{\ivvalue}{\bar \vvalue}
\newcommand{\e}[2][]{{\mathbb E}_{#1}\left[ #2 \right]}
\newcommand{\pr}[2][]{Pr_{#1}\left[#2\right]}
\newcommand{\ind}[1]{\mathbbm 1_{#1}}
\newcommand{\commit}{\text{Commit}}
\newcommand{\poly}{poly}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> macros.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]

\newcommand{\authnote}[2]{{ \footnotesize \bf{\color{red}[#1's Note:
{\color{blue}#2}]}}}

\newcommand{\me}[1]{{\authnote{Meryem} {#1}}}
\newcommand{\mattnote}[1]{{\authnote{Matt} {#1}}}
\newcommand{\madd}[1]{{\color{blue} #1}}
\newcommand{\mc}[1]{{\color{red}MVXF: #1}}
\newcommand{\mattfootnote}[1]{\footnote{\textcolor{blue}{#1}}}
\newcommand{\hide}[1]{}

% Math symbols
\newcommand{\rev}{\text{Rev}}
\newcommand{\vvalue}{\varphi}
\newcommand{\ivvalue}{\bar \vvalue}
\newcommand{\e}[2][]{{\mathbb E}_{#1}\left[ #2 \right]}
\newcommand{\pr}[2][]{Pr_{#1}\left[#2\right]}
\newcommand{\ind}[1]{\mathbbm 1_{#1}}
\newcommand{\commit}{\text{Commit}}
\newcommand{\poly}{poly}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
